Event-Clock Nested Automata

In this paper we introduce and study Event-Clock Nested Automata (ECNA), a formalism that combines Event Clock Automata (ECA) and Visibly Pushdown Automata (VPA). ECNA allow to express real-time properties over non-regular patterns of recursive programs. We prove that ECNA retain the same closure and decidability properties of ECA and VPA being closed under Boolean operations and having a decidable language-inclusion problem. In particular, we prove that emptiness, universality, and language-inclusion for ECNA are EXPTIME-complete problems. As for the expressiveness, we have that ECNA properly extend any previous attempt in the literature of combining ECA and VPA.

==> PreliminariesOld.tex <==
\section{Preliminaries}\label{sec:backgr}

In the following  $\Nat$ denotes  the set of natural numbers and $\RealP$ denotes the set of non-negative real numbers.
%
Let $w$ be a finite or infinite word over some alphabet. We denote by $|w|$ the length of $w$ (we set $|w|=\infty$ if $w$ is infinite). For all  $i,j\in\Nat $, with $i\leq j$, $w_i$ is
$i$-th letter of $w$, while $w[i,j]$ is the finite subword
%of $w$ given by
 $w_i\cdots w_j$.

 An \emph{infinite timed word} $w$ over a finite alphabet $\Sigma$ is
an infinite word $w=(a_0,\tau_0) (a_1,\tau_1),\ldots$ over $\Sigma\times \RealP$ (intuitively, for each $i$, $\tau_i$ is the time at which $a_i$ occurs) such that the sequence $\tau= \tau_0,\tau_1,\ldots$ of timestamps  satisfies: (1) $\tau_i\leq \tau_{i+1}$ for all $i\geq 0$ (monotonicity), and (2) for all $t\in\RealP$, $\tau_i\geq t$ for some $i\geq 0$
(divergence). The timed word $w$ is also denoted by  $(\sigma,\tau)$, where $\sigma$ is the untimed word  given by $a_0 a_1\ldots$ and $\tau$ is the sequence of timestamps. An \emph{$\omega$-timed language} over $\Sigma$ is a set of infinite timed words over $\Sigma$.\vspace{-0.2cm}



\paragraph{Pushdown alphabets and abstract paths.}
A \emph{pushdown alphabet} is
a finite alphabet $\Sigma=\Scall\cup\Sret\cup\Sint$ which is partitioned into a set $\Scall$ of \emph{calls}, a set
$\Sret$ of \emph{returns}, and a set $\Sint$ of \emph{internal
  actions}. The pushdown alphabet $\Sigma$  induces a nested hierarchical structure in a given word over $\Sigma$ obtained by associating
to each call the corresponding matching return (if any) in a well-nested manner. Formally, the set  of \emph{well-matched words} is the set of finite words $\sigma$ over
$\Sigma$ inductively defined as follows:
%
\begin{compactitem}
\item the empty word $\varepsilon$ is well-matched;
\item if $a\in\Sint$ and $\sigma$ is well-mathed, then  $a\cdot \sigma$ is well-matched;
\item  if $c\in\Scall$,
  $r\in\Sret$, and $\sigma,\sigma'$ are well-matched, then $c\cdot \sigma \cdot r \cdot \sigma'$ is well-matched.
\end{compactitem}
%
Fix an infinite word $\sigma$ over $\Sigma$. For a call position $i\geq 0$,
if there is $j>i$ such that $j$ is a return position of $\sigma$ and
$\sigma[i+1,j-1]$ is a well-matched word (note that $j$ is
uniquely determined if it exists), we say that $j$ is the
\emph{matching return} of $i$ along $\sigma$.
For a position $i\geq 0$,
the \emph{abstract successor of $i$ along $\sigma$}, denoted
  $\SUCC(\abs,\sigma,i)$, is defined as follows:
  \begin{compactitem}
  \item If $i$ is a call,  then
    $\SUCC(\abs,\sigma,i)$ is the matching return of $i$ if such a matching return exists; otherwise
     $\SUCC(\abs,\sigma,i)=\NULL$ ($\NULL$ denotes the
    \emph{undefined} value).
  \item If $i$ is not a call, then $\SUCC(\abs,\sigma,i)=i+1$ if $i+1$ is
    not a return position, and $\SUCC(\abs,\sigma,i)=\NULL$, otherwise.
  \end{compactitem}


%

An \emph{abstract path $\nu$} of $\sigma$ is a finite or infinite increasing sequence
of natural numbers $\nu= i_0,i_1,\ldots$ such that
$i_j=\SUCC(\abs,\sigma,i_{j-1})$ for all $1\leq j<|\nu|$. The abstract path $\nu$ is \emph{maximal} (both in the past and in the future)
if there is no abstract path of $\sigma$ having $\nu$ as a proper subsequence.
Intuitively, in the analysis of recursive programs, a maximal  abstract path (\MAP, for short)
captures the local computation within a
procedure removing computation fragments corresponding to nested
calls. Note that for every position $i$ of $\sigma$, there is exactly one maximal abstract path of $\sigma$ visiting
position $i$: we denote by $\Pos(\abs,\sigma,i)$ the set of positions visited by the \MAP\ of $\sigma$ associated with position $i$.

For instance, consider the untimed word $\sigma$ depicted in Figure \ref{fig-word} over the pushdown alphabet $\Sigma$ with $\Scall =\{c\}$, $\Sret =\{r\}$, and $\Sint =\{\i\}$. Let $\sigma$ be $\sigma_p \cdot \i^{\omega}$, where $\sigma_p$ is the prefix  until position $10$ depicted in figure. The \MAP\ visiting position $1$ is the infinite sequence $1,6,7,9,10,11,12,13 \ldots$; the \MAP\ visiting position $0$ consists of just position $0$ since it corresponds with a call devoid of a matching return ($succ(a,\sigma,0)=\NULL$); the MAP visting position $2$ is the sequence $2,3,5$ and the one visting $4$ consists of iust position $4$.

\input{Figure1}
\vspace{-0.6cm}

\section{Event-clock nested automata}


In this section we define the formalism of \emph{Event-clock Nested Automata} (\ECNA), which allow the combined used of event clock and visible operations on the stack. To this end, we augment the standard set of event clocks with a set of \emph{abstract event clocks} which measure the time elapsed since the last occurrence (resp., the time to wait for the next occurrence) of the associated event along the maximal abstract path of the given timed word visiting the current position.


In the following, we fix a pushdown alphabet $\Sigma=\Scall\cup\Sret\cup\Sint$. We associate with each symbol $b\in \Sigma$, four event clocks:
the \emph{global recorder clock $x_b$} (resp. the \emph{global predictor clock $y_b$}) recording the time elapsed since the last occurrence of $b$ if any
(resp. the time required to the next occurrence of $b$ if any);  the \emph{abstract recorder clock $x_b^{\abs}$} (resp. the \emph{abstract predictor clock $y_b^{\abs}$}) recording the time elapsed since the last occurrence of $b$ if any (resp. the time required to the next occurrence of $b$) in the abstract path including the current position. Given an infinite timed word over $\Sigma$,
the values of the clocks in a fixed position of the word can be deterministically determined as follows.

\begin{definition}[Event clocks and determinisitic clock valuations] \emph{The set $C_{\Sigma}$ of event clocks associated
with $\Sigma$ is given by $C_{\Sigma}:= \bigcup_{b\in\Sigma} \{x_b,y_b,x_b^{\abs},y_b^{\abs}\}$.
A \emph{clock valuation} over $C_{\Sigma}$ is a mapping $\val: C_{\Sigma} \mapsto \RealP\cup \{\NULL\}$, assigning to each event clock a value in
$\RealP\cup \{\NULL\}$.
 %where $\NULL$ denotes the \emph{undefined} value.
Given an infinite timed word $w=(\sigma,\tau)$ over
 %the pushdown alphabet
 $\Sigma$ and a position $i$, the \emph{clock valuation $\val^{w}_i$ over $C_{\Sigma}$}, specifying the values of the event clocks at position $i$ along $w$, is defined as follows for each $b\in\Sigma$:}
%
\[
\begin{array}{l}
\val^{w}_i(x_b)  =  \left\{
\begin{array}{ll}
\tau_i - \tau_j
&    \text{ if } \exists j<i:\, b= \sigma_j,  \text{ and }\, \forall k: j < k < i \Rightarrow b\neq  \sigma_k
\\
\NULL
&    \text{ otherwise }
\end{array}
\right. \vspace{0.2cm}\\
\val^{w}_i(y_b)  =  \left\{
\begin{array}{ll}
\tau_j - \tau_i
&    \text{ if } \exists j>i:\, b= \sigma_j,  \text{ and }\, \forall k: i < k < j \Rightarrow b\neq \sigma_k
\\
\NULL
&    \text{ otherwise }
\end{array}
\right. \vspace{0.2cm}\\
\val^{w}_i(x_b^{\abs})  =  \left\{
\begin{array}{ll}
\tau_i - \tau_j
&    \text{ if } \exists j<i:\, b= \sigma_j,\, j\in\Pos(\abs,\sigma,i),  \text{ and}\,
\\
& \,\,\,\,\,\,\forall k: (j < k < i   \text{ and }\, k\in\Pos(\abs,\sigma,i))  \Rightarrow b\neq \sigma_k\\
\NULL
&    \text{ otherwise }
\end{array}
\right.
\vspace{0.2cm}\\
\val^{w}_i(y_b^{\abs})  =  \left\{
\begin{array}{ll}
\tau_j - \tau_i
&    \text{ if } \exists j>i:\, b= \sigma_j,\, j\in\Pos(\abs,\sigma,i),  \text{ and}\,
\\
& \,\,\,\,\,\,\forall k: (i < k < j   \text{ and }\, k\in\Pos(\abs,\sigma,i))  \Rightarrow b\neq \sigma_k\\
\NULL
&    \text{ otherwise }
\end{array}
\right.
\end{array}
\]
\end{definition}

%Thus, at position $i$ of the given  word, the value of the global recorder clock $x_b$ is the time since the last occurrence of symbol $b$
%if such an occurrence exists and it undefined otherwise; symmetrically,
%the value of the global predictor clock $y_b$ is the time to wait for  the next occurrence of $b$ if such an occurrence exists and it undefined otherwise.
Notice that the values of the abstract recorder clock $x_b^{\abs}$ and the abstract predictor clock $y_b^{\abs}$ are not immediately defined in the timed word $w$ as the global clocks but with respect to the \MAP\ of $w$ visiting the current valuation position.


For  $C\subseteq C_{\Sigma}$ and a clock valuation
$\val$ over $C_{\Sigma}$, $\val_{\mid C}$ denotes the restriction of $\val$ to the set $C$.
 A \emph{clock constraint} over $C$ is a conjunction of atomic formulas of the form
$z \in I$, where $z\in C$, and
$I$ is either an interval in $\RealP$ with bounds in $\Nat\cup\{\infty\}$, or the singleton $\{\NULL\}$ (also denoted by $[\NULL,\NULL]$).
For a clock valuation $\val$ and a clock constraint $\theta$, $\val$ satisfies $\theta$, written
$\val\models \theta$, if for each conjunct $z\in I$ of $\theta$, $\val(z)\in I$. We denote by $\Phi(C)$ the set of clock constraints over $C$.


For technical convenience, we first introduce an extension of the known class of \emph{Visibly Pushdown Timed Automata} (\VPTA) \cite{BouajjaniER94,EmmiM06},
called \emph{nested} \VPTA. Nested \VPTA\ are simply \VPTA\ augmented with event clocks. Therefore, transitions of \emph{nested} \VPTA can constrained over a pair of disjoint finite set of clocks: a finite set of standard clocks $C_{st}$ and the disjoint set $C_{\Sigma}$ of event clocks. As usual, standard clocks can be reset and the valuation of a clock on a position of a word depends in general on the behaviour on the automaton and not only, as for event clocks, on the word.

The class of Event Clock Nested Automata correspond to the subclass of nested \VPTA\ where the set of standard clocks  $C_{st}$ is empty.

%Let $C_{st}$ be a finite set of standard clocks disjunct from $C_{\Sigma}$.
 A (standard) clock valuation over $C_{st}$ is a mapping $\sval: C_{st} \mapsto \RealP$ (note that the undefined value $\NULL$ is not admitted). For $t\in\RealP$ and a reset set $\Res\subseteq C_{st}$, $\sval+ t$ and $\sval[\Res]$ denote  the  valuations over $C_{st}$ defined as follows for all $z\in C_{st}$: $(\sval +t)(z) = \sval(z)+t$, and $\sval[\Res](z)=0$ if $z\in \Res$ and $\sval[\Res](z)=\sval(z)$ otherwise.
For $C\subseteq C_\Sigma$ and a valuation $\val$ over $C$, $\val\cup \sval$ denotes the valuation over $C_{st}\cup C$ defined in the obvious way.


\begin{definition}[Nested \VPTA]\emph{ A B\"{u}chi \emph{nested} \VPTA\   over  $\Sigma= \Scall\cup \Sint \cup \Sret$ is a tuple
$\Au=\tpl{\Sigma, Q,Q_{0},D=C\cup C_{st},\Gamma\cup\{\top\},\Delta,F}$, where $Q$ is a finite
set of (control) states, $Q_{0}\subseteq Q$ is a set of initial
states, $C\subseteq C_{\Sigma}$ is a set of event clocks, $C_{st}$ is a set of standard clocks disjunct from $C_{\Sigma}$, $\Gamma\cup\{\top\}$ is a finite stack alphabet,  $\top\notin\Gamma$ is the special \emph{stack bottom
  symbol}, $F\subseteq Q$ is a set of accepting states, and $\Delta_c\cup \Delta_r\cup \Delta_i$ is a transition relation, where ($D= C\cup C_{st}$):
  \begin{compactitem}
    \item $\Delta_c\subseteq Q\times \Scall \times \Phi(D) \times 2^{C_{st}} \times Q \times \Gamma$ is the set of \emph{push transitions},
    \item $\Delta_r\subseteq Q\times \Sret  \times \Phi(D) \times 2^{C_{st}} \times (\Gamma\cup \{\top\}) \times Q $ is the set of \emph{pop transitions},
       \item $\Delta_i\subseteq Q\times \Sint\times \Phi(D) \times 2^{C_{st}} \times Q $ is the set of \emph{internal transitions}.
  \end{compactitem}}
\end{definition}


 We give now the intuition of the behavior of a Nested \VPTA $\Au$. Assume that reading the $i$-th position of $w$ the current control state of $\Au$ is $q$,  $\val^{w}_i$ is the event-clock valuation associated with  $w$ at  position $i$,  $\sval$ is the current valuation of the standard clocks in $C_{st}$, and $t=\tau_i-\tau_{i-1}$ is the time elapsed from the last transition (let in the following $\tau_{-1}=0$).
On reading  a call $c\in \Scall$,  $\Au$ chooses a push transition of the
form $(q,c,\theta,\Res,q',\gamma)\in\Delta_c$ fulfilling the constraint $\theta$ by  valuation $(\sval+t)\cup (\val^{w}_i)_{\mid C}$,  pushes the symbol $\gamma\neq \bot$ onto the
stack, resets the standard clocks in  $\Res$, and the control changes from $q$ to $q'$.
On  reading a return $r\in\Sret$,  $\Au$ chooses a pop transition of the
form $(q,r,\theta,\Res,\gamma,q')\in\Delta_r$ such taht $\gamma$ is the symbol on top of the stack and $\theta$ is fulfilled  by $(\sval+t)\cup (\val^{w}_i)_{\mid C}$,  pops $\gamma$ from the stack (if $\gamma=\bot$, then $\gamma$ is read but not removed),  resets the standard clocks in $\Res$  and the control changes from $q$ to $q'$.
Finally, on reading an internal action $a\in\Sint$, $\Au$ chooses an internal transition of the
form $(q,a,\theta,\Res, q')\in\Delta_i$ fulfilling the constraint $\theta$  by $(\sval+t)\cup (\val^{w}_i)_{\mid C}$, resets the standard clocks in $\Res$,
and the control changes from $q$ to $q'$ without affecting the stack.

A configuration of $\Au$ is a triple $(q,\beta,\sval)$, where $q\in Q$ is the control state,
$\beta\in\Gamma^*\cdot\{\top\}$ is the stack content, and $\sval$ is the valuation over $C_{st}$.
A run $\pi$ of $\Au$ over an infinite timed word $w=(\sigma,\tau)$ on $\Sigma$ is an infinite sequence $\pi$ of configurations
 $\pi=(q_0,\beta_0,\sval_0),(q_1,\beta_1,\sval_1),\ldots
$ such that $q_0\in Q_{0}$,
$\beta_0=\top$, $\sval_0(z)=0$ for all $z\in C_{st}$ (initialization requirement), and for all $i\geq 0$ and $t_i=\tau_i-\tau_{i-1}$, it  holds:
%
\begin{itemize}
\item \textbf{Push:} If $\sigma_i \in \Scall$, then for some $(q_i,\sigma_i,\theta,\Res,q_{i+1},\gamma)\in\Delta_c$,
  $\beta_{i+1}=\gamma\cdot \beta_i$, $\sval_{i+1}= (\sval_i +t_i)[\Res]$,  and $(\sval_i +t_i)\cup(\val^{w}_i)_{\mid C}\models \theta$.
%
\item \textbf{Pop:} If $\sigma_i \in \Sret$, then for some
  $(q_i,\sigma_i,\theta,\Res,\gamma,q_{i+1})\in\Delta_r$, $\sval_{i+1}= (\sval_i +t_i)[\Res]$, $(\sval_i +t_i)\cup(\val^{w}_i)_{\mid C}\models \theta$,  and \emph{either}
  $\gamma\neq\bot$ and $\beta_{i}=\gamma\cdot \beta_{i+1}$, \emph{or}
  $\gamma=\beta_{i}= \beta_{i+1}=\top$.
%
\item \textbf{Internal:} If $\sigma_i \in \Sint$, then for some
  $(q_i,\sigma_i,\theta,\Res,q_{i+1})\in\Delta_i$, $\beta_{i+1}=\beta_i$, $\sval_{i+1}= (\sval_i +t_i)[\Res]$, and $(\sval_i +t_i)\cup(\val^{w}_i)_{\mid C}\models \theta$.
\end{itemize}
%
The run $\pi$ is \emph{accepting} if  there are infinitely many positions $i\geq 0$ such that $q_i\in F$.
The \emph{timed language} $\TLang(\Au)$ of $\Au$ is the set of infinite timed words $w$ over $\Sigma$
 such that there is an accepting run of $\Au$ on $w$. The \emph{greatest constant of $\Au$}, denoted $K_\Au$, is the greatest natural number used as bound in some clock constraint of $\Au$.
For technical convenience, we also consider nested \VPTA\ equipped with a \emph{generalized B\"{u}chi acceptance condition} $\mathcal{F}$ consisting of a family of sets of accepting states. In such a setting, a run $\pi$ is accepting if for each B\"{u}chi component $F\in \mathcal{F}$, the run $\pi$ visits infinitely often states in $F$.

  A \VPTA\ \cite{EmmiM06} corresponds to  a nested \VPTA\ whose set $C$ of event clocks is empty.
An \emph{\ECNA} is a  nested \VPTA\ whose set $C_{st}$ of standard clocks is empty. For
\ECNA, we can omit the reset component $\Res$ from the transition function and the valuation component $\sval$ from each configuration
$(q,\beta,\sval)$. Note the the class of \ECVPA\ corresponds to the subclass of  \ECNA\ where abstract event-clocks are disallowed.
We also consider two additional subclasses of \ECNA: \emph{abstract predicting} \ECNA\ (\APCNA, for short) which do not use  abstract recorder clocks,
and \emph{abstract recording} \ECNA\ (\ARCNA, for short) which do not use  abstract predictor clocks. Note that both
\APCNA\ and \ARCNA\ subsume \ECVPA.




\begin{example}\label{example:ECNA} Let us consider the abstract recording \ARCNA\ in Figure \ref{arcna}, with $\Scall =\{c\}$, $\Sret =\{r\}$, and $\Sint=\{a,b,\i\}$. The transition relation ensures that
for each accepted word, the \MAP\ visiting the $b$-position associated with the transition $\delta$ from $q_4$ to $q_5$ cannot visit the $a$-positions following the call positions. This implies that the valuation of
$x^{\abs}_{a}$ in  $\delta$ is defined only if the visited  occurrences of calls $c$ and returns $r$ are perfectly matched.
% (i.e. the visited prefix of the word is well matched).
Hence, the  abstract recorder constraint $x^{\abs}_{a}=1$ on the transition from $t$ ensures that the accepted language $\TLangRec$  consists of all the timed words of the form $(\sigma,\tau)\cdot (\i^{\omega},\tau')$ such that $\sigma$ is a well-matched word of the form $a \cdot c^{+} \cdot a^{+} \cdot r^{+} \cdot b^{+}$ and the time difference in $(\sigma,\tau)$  between the first and last symbols is $1$, i.e. $\tau_{|\sigma|-1}-\tau_0=1$. The example shows that $\ECNA$ allow to express a meaningful property of recursive systems, namely the ability of bounding the time required to perform an internal activity cosnsisting of an unbounded number of procedural recursive calls (and returns).

\input{Figure2.tex}

\vspace{-0.2cm}
Similarly, it is easy to define an abstract predicting \APCNA\ accepting the timed language  $\TLangPred$ consisting of all the timed words of the form $(\sigma,\tau)\cdot (\i^{\omega},\tau')$ such that $\sigma$ is a well-matched word of the form $a^{+}  \cdot  c^{+} \cdot b^{+} \cdot r^{+} \cdot b$ and the time difference in $(\sigma,\tau)$  between the first and last symbols is $1$.
\end{example}


\paragraph{Closure properties of B\"{u}chi \ECNA.} As stated in the following theorem, the class of languages accepted by B\"{u}chi \ECNA\ is closed under Boolean operations. The proof exploits a technique similar to that used in~\cite{TangO09} to prove the analogous property for \ECVPA\ (for details, see Appendix~\ref{APP:closureProperties}).

 \newcounter{theo-closureProperties}
\setcounter{theo-closureProperties}{\value{theorem}}


 \begin{theorem}\label{theorem:closureProperties} The class of $\omega$-timed languages accepted by B\"{u}chi
\ECNA\ is closed under union, intersection, and complementation. In particular, given two  B\"{u}chi
\ECNA\ $\Au=\tpl{\Sigma, Q,Q_{0},C,\Gamma\cup\{\top\},\Delta,F}$  and $\Au '=\tpl{\Sigma, Q',Q'_{0},C',\Gamma'\cup\{\top\},\Delta',F'}$ over $\Sigma_\Prop$, one can contruct
\begin{compactitem}
  \item a B\"{u}chi \ECNA\ accepting $\TLang(\Au)\cup \TLang(\Au')$ with $|Q|+|Q'|$ states, $|\Gamma|+|\Gamma'|+1$ stacks symbols, and greatest constant $\max(K_{\Au},K_{\Au'})$;
    \item a B\"{u}chi \ECNA\ accepting $\TLang(\Au)\cap \TLang(\Au')$ with $2|Q||Q'|$ states, $|\Gamma|
    |\Gamma'|$ stacks symbols,  and greatest constant $\max(K_{\Au},K_{\Au'})$;
      \item a B\"{u}chi \ECNA\ accepting the complement of $\TLang(\Au)$ with $2^{O(n^{2})}$ states,  $O(2^{O(n^{2})}\cdot |\Scall|\cdot |\Const|^{O(|\Sigma|)})$ stack symbols, and greatest constant
      $K_\Au$, where $n=|Q|$ and $\Const$ is the set of constants used in the clock constraints of $\Au$.
\end{compactitem}
\end{theorem}

\paragraph{Expressiveness results.} In this section we summarize the expressiveness results for \ECNA. First of all, the languages $\TLangRec$ and $\TLangPred$ defined in Example~\ref{example:ECNA} and accepted by an \ARCNA\ and \APCNA, respectively,  can be used to prove that the subclasses \ARCNA\ and \APCNA\ are uncomparable and strictly included into \ECNA. The basic fact is stated in Proposition \ref{prop:expressivenessPredRec} and proved in Appendix~\ref{APP:expressivenessPredRec}.

As for \ECNA, we have that they are less expressive than B\"{u}chi \VPTA. In fact, by Theorem~\ref{theorem:FromECNAtoVPTA} in Section~\ref{sec:DecisionProcedures}, B\"{u}chi \ECNA\ can be converted into equivalent B\"{u}chi \VPTA\ showing inclusion. The inclusion is strict since, while  B\"{u}chi \ECNA\ are closed under complementation (Theorem~\ref{theorem:closureProperties}),   B\"{u}chi \VPTA\ are not~\cite{EmmiM06}.

Finally, we can compare \ECNA\ with  \ECVPA. In~\cite{BhaveDKPT16}, an equally-expressive extension of \ECVPA\ over finite words,  by means of a \emph{timed} stack, is investigated. The B\"{u}chi version of
	such an extension can be trivially encoded in  B\"{u}chi \ARCNA. Moreover, the proof of Proposition~\ref{prop:expressivenessPredRec} can also be used to prove that
	B\"{u}chi  \ECVPA\ with timed stack are less expressive than both B\"{u}chi \ARCNA\ and B\"{u}chi \APCNA.
	
The general picture of the expressiveness results is summarized by Theorem\ref{th:express}. Note that the listed  results also hold for the automata version over finite words.



 \newcounter{prop-expressivenessPredRec}
\setcounter{prop-expressivenessPredRec}{\value{proposition}}


\begin{proposition}\label{prop:expressivenessPredRec} The timed language $\TLangRec$ (resp., $\TLangPred$) is \emph{not} definable by an abstract-predicting (resp., abstract-recording) B\"{u}chi \ECNA.
Moreover, the language $\TLangRec\cup \TLangPred$ is not definable neither by an  abstract-predicting  B\"{u}chi \ECNA\ nor
by an abstract-recording B\"{u}chi \ECNA.
\end{proposition}

%By Theorem~\ref{theorem:FromECNAtoVPTA} in Section~\ref{sec:DecisionProcedures}, B\"{u}chi \ECNA\ can be converted into equivalent B\"{u}chi \VPTA. However, while  B\"{u}chi \ECNA\ are closed under complementation (Theorem~\ref{theorem:closureProperties}),   B\"{u}chi \VPTA\ are not~\cite{EmmiM06}. By Example~\ref{example:ECNA}, $\TLangRec$ is  definable by a B\"{u}chi  abstract-recording \ECNA\ (\ARCNA) and
%$\TLangPred$ is  definable by a B\"{u}chi  abstract-predicting \ECNA\ (\APCNA). Thus, by Proposition~\ref{prop:expressivenessPredRec}, we obtain the following relationships between the considered classes of automata (for brevity, in the following theorem, we omit the prefix B\"{u}chi). Note that the following expressiveness results also hold for the automata version over finite words.

\begin{theorem}\label{th:express}The following holds:\vspace{-0.2cm}
\[
\begin{array}{ll}
  (1) \,\, \APCNA \not\subseteq \ARCNA   &  \quad (2) \,\, \ARCNA \not\subseteq \APCNA   \\
  (3) \,\, \ECVPA \subset \ARCNA          & \quad  (4) \,\, \ECVPA \subset \APCNA \\
  (5) \,\, \APCNA \cup \ARCNA \subset  \ECNA  & \quad (6)\,\, \ECNA   \subset \VPTA
\end{array}
\]
\end{theorem}


%\begin{remark} In~\cite{BhaveDKPT16}, an equally-expressive extension of \ECVPA\ over finite words,  by means of a \emph{timed} stack, is investigated. The B\"{u}chi version of
%such an extension can be trivially encoded in  B\"{u}chi \ARCNA. Moreover, the proof of Proposition~\ref{prop:expressivenessPredRec} can also be used for showing that
%B\"{u}chi  \ECVPA\ with timed stack are less expressive than both B\"{u}chi \ARCNA\ and B\"{u}chi \APCNA.
%\end{remark} 
